Compressive Neural Representations of Volumetric Scalar Fields

We present an approach for compressing volumetric scalar fields using implicit neural representations. Our approach represents a scalar field as a learned function, wherein a neural network maps a point in the domain to an output scalar value. By setting the number of weights of the neural network to be smaller than the input size, we achieve compressed representations of scalar fields, thus framing compression as a type of function approximation. Combined with carefully quantizing network weights, we show that this approach yields highly compact representations that outperform state-of-the-art volume compression approaches. The conceptual simplicity of our approach enables a number of benefits, such as support for time-varying scalar fields, optimizing to preserve spatial gradients, and random-access field evaluation. We study the impact of network design choices on compression performance, highlighting how simple network architectures are effective for a broad range of volumes.

==> first_round_reviews.tex <==
Reviews of 1127 Neural Volume Compression using Implicit Representations

Reviewer 4 (coordinator)

Summary Review Text

All reviewers agree that the paper presents a new compression approach on machine learning that is of high interest to the EuroVis conference audience. While the approach is computationally very expensive, this limitation is communicated honestly in the paper and the new approach has the potential to create new research ideas in visualization. Thus, all reviewers recommend accepting the paper.

To be published, the following minor revisions are necessary:

* Include the information provided in the rebuttal in the camera ready version of the paper as it clarifies important issues.
* Extend the description of the used neural network architecture (R4, R3) and improve Figure 2 to go along with it. In particular, this description should not require reading the SIREN paper (or any other references) and all relevant equations should appear in the paper.
* Clarify mathematical notation (R4).
* Add the reference suggested by R1 (Foundations of Multivariate Functional Approximation for Scientific Data) to related work
* Add more details about choosing parameters to the paper (R2, already partially in the rebuttal, a few more details would be helpful).
* While cropping uses the original input data, it may change complexity (by picking a particularly complex or simple region). A few sentences discussion about the effects would be helpful (R3).

----Additional rebuttal comments from the primary------

The comments in the rebuttal phase were helpful to understand the paper.

The overall rating remains a week consensus to accept the paper.



There are two responses to the rebuttal document:

W2: I still contradict the authors in the mathematical phrasing as I am still the opinion that the authors define a neural network that is parameterized by an implicit function and do not represent the field as an implicit function that is parameterized by a neural network.
Especially because the implicit function is given in [SMB*20] Eq. 1 and never in the current paper. (cf. Teaser image and Section 3).
After the explanation, I agree with the authors, that f - as defined in the paper - is indeed defined as an implicit function if considering [SMB*20]s implicit equation.

W2: Visual representations are good to have but always lack errors due to the representation, therefore, other statistics may always help. Especially because in data visualization, the data quality required for some algorithms (especially based on derivatives) may be finer grained than the graphical representation.

Paper Type

Algorithm / Technique

References

At large, all important references are included

Utility, Importance (relevance in general)

Possibly useful

Soundness (technical soundness, soundness of approach)

Some concerns on correctness, some choices questionable

Reproducibility

Many issues discussed, but some important details left out

Presentation Quality

Fair: some structural changes or some wordsmithing needed

Overall Rating

Borderline on the accept side (3.5/5): While this paper is on the borderline, I would vote to accept if forced to choose.

Expertise

Knowledgeable

Paper Short Summary

The paper describes a compression algorithm for 3d scalar fields based on the lossy compression of the parameters of a neural network which provides a lossy approximation of the data.

Paper Strengths

S1: Data compression is an important topic and the authors address this by a novel approach to the visualization community.

S2: The idea may have potential in the future, but, as stated by the authors, it is rather slow at the moment.

S3: Overall, the paper is well written and the method is tested on multiple data sets. Nevertheless, some more tests should be added (see W3)

...

Paper Major Weaknesses

W1: The network design is highly based on a previous design (SIREN). The paper references that paper several times without giving an overview of the main design of SIREN and without summarizing explicitly the differences of the new design. Instead of Figure 2, a more detailed depiction of the network design should be presented.

W2: The mathematical description of the method uses the wrong mathematical terms

W3: As the paper describes two independent compression schemes (by the network and by quantization of the network parameters), I miss a proper evaluation of both independently. Also when speaking of quantization, the data types of the network are required. If the data set is given by 200000 values in 8 Bit and is represented with 1/200 compression as 1000 long double values with 128 Bit the resulting data is only 8% instead of 0,5 of the data set size.

...

The description of the compression method (section 3) is hard to understand. Some mathematical terms are used inappropriate.

Even though f(x,y,z) is later defined similar to an "implicit function" in equation (1), it should not be called implicit function when being introduced. This is also true for the word implicit in the title: The representation with the given neural network is _explicit_. The definition of the function.

The name d-tensor for a field is also misleading, as the representation of the field does not have tensor properties: X does not map vectors to scalars, it is not linear, it does not transform as the coordinate system changes...

The variable names are confusing: m is the number of parameters, but the number of points in the field is defined as capital C.
Paper Minor Issues
M1: Figure 2 is not informative as it does not provide any specific detail of the compression algorithm other than an overview. The right side of the image is structured differently an than the left side as one would expect a visualization of the decompression algorithm.

M2: The decoder is described very rudimentarily. Especially the decoder complexity should be analyzed better.

M3: The runtime of the code is rather slow and not comparable to other compression algorithms. Therefore it is not applicable at the moment.

...

The value lambda in equation 3 has been set to 0.05. Is there a reason for that value? What does it depend on?

Why are the networks compressed with m = C/200?

The decoder is described as some "matrix multiplications followed by sine evaluations" The calculation highly depends on the size of the matrices and the number of sine evaluations. I see the advantage of randomly sampling the field and having an interpolation given by the technique, but evaluating a lot of sine functions may be very slow.

As the field is optimized using the sample points, only, it is important to find out about the behavior of the field between the sample points (this is mentioned explicitly as an advantage of the method in figure 2).

Overall Assessment

The paper is well written and a good contribution. Nevertheless, there are some major issues with the approach that should be studied and presented in the final version of the paper.

Reviewer 3 (committee member)
Paper Type

Algorithm / Technique

References

At large, all important references are included

Utility, Importance (relevance in general)

Possibly useful

Soundness (technical soundness, soundness of approach)

Approach is (technically/mathematically) correct and well justified

Reproducibility

Everything critical is discussed

Presentation Quality

Good: only minor typos and grammar problems

Overall Rating

Borderline on the accept side (3.5/5): While this paper is on the borderline, I would vote to accept if forced to choose.

Expertise

Knowledgeable

Paper Short Summary

The paper presents a new compression approach based on deep learning. This approach considers input data as an implicit function and trains a neural network to reproduce this functions. The parameters of the resulting neural network comprise the compressed representation of the function. The compression ratio can be controlled through the number of parameters in the neural network. The fewer parameters the higher the compression ratio. A by-product of this approach is that the higher the compression ratio, the less computationally expensive the approach becomes. The paper also compares the compression result to another state of the art compression method (TTHRESH).

Paper Strengths

S1: A new approach to compression of scientific data that has the potential to create new research directions in visualization

S2: Comparison to state of the art compression algorithm (TTHRESH)

S3: Method has ability to consider quality of derived quantities (e.g., gradients) during compression

S4: Demonstrated use with visualization algorithms (volume rendering, isosurface extraction)

S5: Thorough and honest discussion of limitations

Paper Major Weaknesses

W1: The method is computationally very expensive (hours per volume). The manuscript envisions use for in situ compression on supercomputers, but the computational cost (at least at the moment) is too high for that purpose as it would slow down a simulation too much.

W2: Comparison to TTHRESH is just based on a single PSNR score. A more thorough comparison (e.g., region based for select data sets) would be desirable.

W3: Control is by compression ratio, difficult to guarantee fixed error bound (which would be a desirable parameter to control for in situ use).

Paper Minor Issues

M1: Description of used neural network architecture should be more detailed (provide a more detailed overview discussion of SIREN). Also, describe in more detail how you enrich SIREN with residual connections). An illustration of the network architecture would help significantly.

M2: Why are you using center crops rather than down-sampled data? How does this affect data complexity. A more thorough discussion of this choice is necessary.

M3: Sentence in Section 3 "where assuming its size $m$ ... requires smaller storage" is difficult to understand and should be rephrased (possibly split into multiple sentences).

M4: What does "ensured stable through a principled initialization scheme" mean? In particular what is a "principled initialization scheme"?

M5: Minor types: 2.1 transformed spaced -> transformed space

M6: Spell out Peak signal-to-noise ratio (PSNR) in first use and provide brief description.

...

Overall Assessment

The paper is well written and addresses an important topic. At the moment the major limitation is the computational cost (runtime), which makes the method impractical for many applications. However, the manuscript presents a new way to think about compression of scientific data, which makes it a valuable contribution to EuroVis. Overall, I recommend accepting the paper.

Reviewer 1 (reviewer)

Paper Type

Algorithm / Technique

References

Some important references are missing

Utility, Importance (relevance in general)

Addresses a clear need

Soundness (technical soundness, soundness of approach)

Approach is (technically/mathematically) correct and well justified

Reproducibility

Everything critical is discussed

Presentation Quality

Excellent: exposition is clear and writing flows well

Overall Rating

Borderline on the accept side (3.5/5): While this paper is on the borderline, I would vote to accept if forced to choose.

Expertise

Knowledgeable

Paper Short Summary

This paper describes the application of the SIREN neural network to compress scientific 3d and 4d data, and benchmarks the compression ratio and PSNR for a variety of datasets commonly evaluated in the visualization community. It further improves the compression ratio by quantizing the weights into a fixed number of bits, and by adding a gradient term to the loss function. The compression and error rates outperform the state of the art tthresh approach, at the expense of long training times customized for each data set.

Paper Strengths

S1: Demonstrating how the SIREN model can serve as a surrogate for a 3d or 4d dataset, with good compression and error metrics. The SIREN method appeared in NeurIPS 2020, which is arguably the top AI conference, but many in the visualization community may not follow it. Sharing that paper in this community by evaluating the compression, with some minor additions such as weight quantization and gradient regularization, has value.

S2: Adding gradient regularization to the loss function to preserve gradients.

S3: Demonstrating good results on a variety of datasets commonly evaluated in the visualization community.

S4: The paper is well written and clear. I found it easy to read and informative.

...

Paper Major Weaknesses

W1: The novelty of the work is incremental, with small additions to the SIREN method. This is the main reason that my score was not higher. The SIREN paper already demonstrated the applicability to implicit representations with examples in scientific computing such as the Poisson, Helmholtz, and wave equations. The current paper benchmarks that technique for compression of sci-vis datasets, and adds small improvements to improve the compressibility and error.

W2:

W3:

...

Paper Minor Issues

M1: I suggest adding geometric B-spline approximation to the related work. [Peterka, T., Nashed, Y., Grindeanu, I., Mahadevan, V., Yeh, R., Tricoche, X.: Foundations of Multivariate Functional Approximation for Scientific Data. Proceedings of IEEE Symposium on Large Data Analysis and Visualization (LDAV) 2018, Berlin, Germany, 2018.] This approach satisfies similar objectives---functional approximation, directly usable without decompressing, able to evaluate points anywhere in the space, able to evaluate high-order derivatives, usable in visualization algorithms---albeit with considerably lower compression and higher error, but trainable in seconds with simple least squares optimization. Not to claim that one method is better than another, only to say that there is another approach to this problem that also is not compression/decompression of the discrete data.

M2:

M3:

...

Overall Assessment

On balance, I think the overall strengths of the paper outweigh the weaknesses, arguing for a weak accept. The presentation quality is very good, and the visualization community needs to know about the SIREN model, which seems to be the best solution for surrogate modeling of scientific data at present. This paper, albeit a little low on novelty, is a good way to exercise the SIREN model on sci-vis datasets by evaluating compression and error rates. Even though I was familiar with SIREN, reading the current paper made me want to employ the technique, and that is a valuable contribution.

Reviewer 2 (reviewer)

Paper Type

Algorithm / Technique

References

At large, all important references are included

Utility, Importance (relevance in general)

Addresses a clear need

Soundness (technical soundness, soundness of approach)

Approach is (technically/mathematically) correct and well justified

Reproducibility

Many issues discussed, but some important details left out

Presentation Quality

Excellent: exposition is clear and writing flows well

Overall Rating

Probably accept (4/5): I would argue for accepting this paper.

Expertise

Knowledgeable

Paper Short Summary

This paper presents a deep-learning-based compression approach of scalar fields defined on regular grids. Specifically, the approach aims to represent an input scalar field as an implicit function, whose parameters are learned/trained for this specific input scalar field. The compression ratio then just follows directly by dividing the number of scalar field samples by the number of network weights (assuming they are stored in the same precision, e.g., floats). This is also the main advantage of the proposed approach, as the compression ratio can directly be controlled by the complexity of the network architecture. Hence, the smaller the number of weights, the better the compression ratio. This has the nice side-effect that using less weights also accelerates training. The authors also demonstrate that their approach can be used to compress multiple scalar fields at once (time-varying data), and that they can improve compression further by using less precise data types for weights in intermediate layers (quantization). The authors also compare their results to a state-of-the-art compression method (TTHRESH), and they show that implicit function representation can directly be used for volume/isosurface visualization (even incorporating gradient information).

Paper Strengths

S1: I really enjoyed reading the paper and it provides a very strong contribution.

S2: The proposed approach provides compression at an architectural level, with the added benefit that training is completed faster for small networks, i.e., high compression ratios.

S3: The authors also compare their results to a state-of-the-art compression method (TTHRESH).

S4: They show that their implicit function representation can directly be used for volume/isosurface visualization (even incorporating gradient information).

Paper Major Weaknesses

(blank)

Paper Minor Issues

M1: The technique depends on multiple parameter and architectural choices that impact the resulting quality, but these can not be determined a prior for a specific input dataset. After reading the paper twice I'm still not able to judge what parameters will give me satisfactory results. Some heuristics are spread around here and there, but I would have preferred a summary guideline to make it easier for people to reproduce the results.

M2: The method inherits all problems of lossy-compression techniques and the AI black-box.

M3: The proposed technique involves long training procedures (as usual for such approaches), but the authors also discuss possible remedies.

M4: By looking at the approach from a distance, representing a scalar field as an implicit function roughly corresponds to smoothing. This is also the reason why it is difficult/impossible to preserve noise with a small number of weights. So the rendering of these smooth representations is pleasing to the eye (as demonstrated by the authors). Although this smoothness is beneficial for visualization, I'm concerned that this has also a drastic (possible damaging) effect on data analysis, which is a problem of all lossy compression techniques. So to me it seems this approach will produce good results for datasets that "already" exhibit "smooth" features, while it will have problems with more discrete features (the foot dataset is actually relatively smooth compared to other bio-medical datasets). This could be discussed in more detail in the conclusion.

M5: In Figure 7 for the asteroid dataset it looks like noise starts to appear in the regions which should be 0 as the compression ratio increases. It was my intuition that implicit functions will preserve such "flat" regions while introducing errors in regions where it is now no longer possible to accurately differentiate between scalar values (see W3: smoothness). So my question is if certain weights can have a global impact, or if they are somewhat locally constraint.

Overall Assessment

Overall, I think the paper is of high quality and only requires minor revisions in the form of further discussions.
